A Modular Formalization of Reversibility for Concurrent Models and Languages

Causal-consistent reversibility is the reference notion of reversibility for concurrency. We introduce a modular framework for defining causal-consistent reversible extensions of concurrent models and languages. We show how our framework can be used to define reversible extensions of formalisms as different as CCS and concurrent X-machines. The generality of the approach allows for the reuse of theories and techniques in different settings.

==> eptcsdata.tex <==
\providecommand{\firstpage}{98}
\providecommand{\publicationstatus}{M. Bartoletti, L. Henrio, S. Knight, and H. T. Vieira (Eds.):\\9th Interaction and Concurrency Experience (ICE 2016)\\
EPTCS 223, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.223.7}{10.4204/EPTCS.223.7}}
\pdfoutput=1

